A first proof of principle booster setup for the MADMAX dielectric haloscope

Axions and axion-like particles are excellent low-mass dark matter candidates. The MADMAX experiment aims to directly detect galactic axions with masses between $40\,\mu{\rm eV}$ and $400\,\mu{\rm eV}$ by using the axion-induced emission of electromagnetic waves from boundaries between materials of different dielectric constants under a strong magnetic field. Combining many such surfaces, this emission can be significantly enhanced (boosted) using constructive interference and resonances. We present a first proof of principle realization of such a booster system consisting of a copper mirror and up to five sapphire disks. The electromagnetic response of the system is investigated by reflectivity measurements. The mechanical accuracy, calibration process of unwanted reflections and the repeatability of a basic tuning algorithm to place the disks are investigated. We find that for the presented cases the electromagnetic response in terms of the group delay predicted by one-dimensional calculations is sufficiently realized in our setup. The repeatability of the tuning is at the percent level, and would have small impact on the sensitivity of such a booster.

==> chap/__zdelete_05results.tex <==
\begin{comment}
	Figure: long term stab, hysteresis, temperature


Repeated measurements of the group delay give direct implications on the stability of the system and accuracy of the mechanical components.

By not moving the disks for around $\sim 15$ hours, we investigated the temporal stability. 
%
The frequency stability of a single observed group delay peak was on the order of $\pm\,\SI{2}{\mega\hertz}$. This corresponds to an uncertainty in disk position of less than a micrometer. The variations are attributed to mechanical vibration or thermal contraction in the setup. Compared to the envisioned boost factor bandwidth of \SI{50}{\mega\hertz}, this indicates that long-term stability of the system is sufficient even under without active vibrational damping and with temperature fluctuations of the order $\pm \SI{1}{\degreeCelsius}$.


\begin{figure}[tb]
	\centering
	\includegraphics[width=0.48\linewidth]{pics/proofofprinciple_booster_position-reproducability-title.pdf}
	\includegraphics[width=0.48\linewidth]{pics/proofofprinciple_booster_boostfactor-reverse-reproducability-title.pdf}
	\caption[Boost Factor Reproducability]{Reproducibility of fit results. \textbf{Left:} Motor position offsets $d_i$ after fitting the physical disk positions such that the measured group delay matches the simulation. \textbf{Right:} Boost factor amplitude and position variation after fitting the model to each of the measured group delays corresponding to the data points in the left plot.}
	\label{fig:seed-setup-reproducabilities}
\end{figure}

The configuration of physical disk positions is found by matching the group delay of the system to the prediction of the 1D model.
To this end optimization schemes need to be employed, minimizing the number of function evaluations -- corresponding to a realignment of the setup and measurement of the electromagnetic response -- while avoiding convergence in local minima.
%
Simple implementations of a genetic \cite{genetic-algorithm} and Nelder-Mead \cite{nelder-mead} algorithm have been tested. The convergence criterion requires changes of the motor positions of less than a $\si{\micro\metre}$.
Fig.~\ref{Fig:4_disk_exemplary}~(right) shows a typical group delay fit for a case of 4 equidistant disks at \SI{7}{mm} distance. 
%
For disk spacings of \SI{8}{\milli\metre}  the situation corresponds to a maximal power boost of $\sim 700$ at a frequency of $\approx \SI{22.4}{\giga\hertz}$ with a FWHM of $\sim \SI{180}{\mega\hertz}$.
While the Nelder-Mead algorithm converges significantly faster, the genetic algorithm seems to be less prone to converge to local minima. 
Fig.~\ref{fig:seed-setup-reproducabilities} shows the distribution of motor positions after repeating the optimization multiple times. While the repeatability in single spacings is better than $\sim \SI{40}{\micro\metre}$, the electromagnetic response is degenerate in the disk spacings, such that higher disk separations at the one end can be partially compensated by smaller spacings on the other end of the booster.
To infer the effect on the power boost factor, the disk positions in the model are optimized such that the model predicts the various measured group delays. The change in frequency and power boost are outlined in Fig.~\ref{fig:seed-setup-reproducabilities}, being $\Delta \beta^2_{\rm max} \approx \SI{10}{\percent}\,\beta^2_{\rm max}$ and $\Delta f \approx \SI{10}{\percent}\,{\rm FWHM}$. We conclude that our system can be aligned to match the predicted response and achieve the desired boost factors within acceptable accuracy for up to 5 disks at equidistant spacings of 6 to 9 mm. A more detailed paper on this setup is in preparation.
\end{comment}


	\subsection{Mechanical Stability and Accuracy}
	\label{sec:results:setup-accuracy}
	\begin{itemize}
		\item group delay can be used to measure mechanical stability, temperature effects, hysteresis, etc.
		\item results of these measurements
		\item other expected effects (misalignment of rails e.g.), discussed later after detailed discussion of the model
	\end{itemize}
	
	\begin{comment}
	
	
	The mechanical stability of the system was investigated by observing the stability of the resonant group delay peak of a single disk and mirror system. Observations over more than a day without moving any motors revealed a temperature dependence of the disk position of around \SI[separate-uncertainty = true]{-7(2)}{\micro \meter \per \kelvin} corresponding to a group delay shift of around $\sim \SI{2}{\mega\hertz \per \kelvin}$, which when accounted for leave the group delay peak stable within $< \SI{100}{\kilo\hertz}$ limited by seismic constrains.
	
    The disk alignment is limited by the accuracy of the precision motors. Using the same measurement strategy but repeatedly moving the precision motors to the same position and taking into account mechanical hysteresis, the group delay peak position is reproduced within a standard deviation of $\sim \SI{1.5}{\mega\hertz}$ corresponding to position errors of the order of  $\sim \SI{700}{\nano\metre}$.
This is still well below the needed accuracy even for larger scale boosters \cite{Brun:2019lyf}.
	
	\end{comment}
	
	\subsection{1D Model Reflection Systematic}
	\label{sec:results:model-accuracy}
	
	\begin{comment}
	
	[TODO check back with jacobs thesis and the actual data we got]
	
	 In order to check the systematics introduced by reflections, we measure the reflectivity of a system with a single disk and mirror at various different distances to the antenna over a range of $\sim \SI{70}{\centi\metre}$. Afterwards, we fit the disks positions in the model. Fig.~\ref{fig:model:gd-incl-reflection}\,(c) shows the fitted disk separation over set distance to the antenna. While long range trends over $\sim todo$ are most likely to be attributed to rail misalignment and are irrelevant for small motor displacements, short range fluctuations $\sim $ are different for the various kinds of reflection models, showing the systematic effect on the disk spacing introduced by the model to be of the order of \SI{10}{\micro\metre}. Such displacements are negligible for our 5 disk boost factors as we will see in the next section.
	
	\end{comment}
	\begin{itemize}
		\item measurement with moving cu disk:
		\subitem rail misalignment (smooth trends)
		\subitem model systematics (wiggles)
	\end{itemize}	
	
	\subsection{Boost Factor Tuning} %Optimization Algorithms and Setup Reproducibility
	\label{sec:results:optim}
	\begin{itemize}		
		\item optimization runs
		\subitem accuracy of fitting algorithm
		\subitem for the various cases: repeatability measurements for fits
		\subitem a plot of what happens in the model if we change it according to the anti-correlation
		\subitem a plot what happens if we uniformly sweep through disk spacing config
	%\end{itemize}	
	%\subsection{Boost Factor}
	%\label{sec:results:bf}
	%\begin{itemize}		
		\item optimization runs
		\subitem consequence for the accuracy at which a certain boost factor can be achieved
		\subitem sensitivity with 300K and 10K system noise temperature
	\end{itemize}
	

%proposed by the algorithm are less than \SI{1}{\micro\metre} from the previous positions.
%Fig.~\ref{fig:pop:tuning}\,(a) shows the result of running the frequency tuning procedure for the same calculated boost factor for 200 times. The correlations among the final disk positions indicate that there exists degeneracy in the disk position phase space. Fig.~\ref{fig:pop:tuning}\,(b) shows the standard deviation of the final disk positions in the case of 1-5 discs. Due to the phase-space degeneracy, the repeatability of the disk spacings deteriorates as the number of discs increases; it rises above \SI{50}{\micro\metre} for five disks.

%We demonstrate a naive tuning of a realistic setup by optimizing the physical disk spacings until the measured reflectivity matches the prediction from the model.
%%The configuration of physical disk positions is found by matching the group delay of the system to the prediction of the 1D model.
%%The objective function (error function) in this case is the the sum of the squared differences %$\chi^2$ between the measured and desired group delay.
%%Therefore, each objective function evaluation now corresponds to a realignment of disk positions and measurement of the reflectivity.
%In order to make this tuning efficient we seek for gradient-free optimization schemes, which minimize the number of objective function evaluations, i.e., realignments of the disk positions.
%On the other hand, it is important to avoid convergence into local minima, e.g. cases in which only a subset of the group delay peaks is fitted correctly.
%
%We consider simple implementations of the genetic~\cite{Whitley1994}, Simulated Annealing~\cite{Laarhoven:1987:SAT:59580} and Nelder-Mead~\cite{Lagarias1998} algorithms.
%%While for the genetic algorithm disk spacings are randomly changed on a dither scale $d$ until no better candidate can be found and $d$ is reduced, Simulated~Annealing is designed to be more resistant against local minima, because it also randomly searches around disk spacings giving an increase of the error function. The probability to go to disk spacings increasing the error function is parametrized by a temperature $T$, which is being gradually decreased.
%%Nelder-Mead is a more deterministic approach, where the next solution is selected by considering a simplex of $N+1$ previous solutions, where $N$ is the dimension of the problem, i.e., in our case the number of disk spacings.
%As a convergence criterion we require for all algorithms changes of the motor positions of less than a $\si{\micro\metre}$.
%While they perform similar in terms of number of function evaluations, Nelder-Mead and Simulated Annealing appear to avoid local minima better for our problem.

	\begin{comment}
Fig.~\ref{fig:pop:tuning}\,(a,b) shows results of running the frequency tuning procedure the same calculated boost factor with four disks for $\sim 200$ times: In (a) we histogram the final motor positions.
The correlations among the final disk positions indicate that there exists degeneracy in the disk position phase space.
(b) shows the standard deviation of the final disk positions in the case of $1-5$ disks. Due to the phase-space degeneracy, the repeatability rapidly deteriorates with disk number, raising above \SI{50}{\micro\metre} for 5 disks.
%An important reason for this increase is found in the degenerate minima of the optimizations, leading to correlations in the solution space of disk spacings.

In order to quantify the the systematic uncertainty on the boost factor arising from tuning,
we use the same optimization algorithm, but now change the disk positions in the model instead of the setup, such that the calculated group delays match the measured group delays.
This is repeated for each set of final disk spacings in the aforementioned tuning procedure, and the boost factor is calculated for each set of disc positions in the model. The systematic uncertainty of the boost factor is then extracted from this ensemble of calculated boost factors, thus taking into account the effect of disk spacing degeneracy.
%we re-optimize the disk spacings in the model instead of the setup for each of the previous optimization result, until all the measured group delays are reproduced in the model. This gives a prediction on the boost factor for each optimization, allowing us to determine how well the tuning can reproduce the same boost factor position and amplitude.
Fig.~\ref{fig:pop:tuning}\,(c) shows the uncertainties on the boost factor center frequency and amplitude as a function of the number of disks. The frequency error ($< \SI{2}{\mega\hertz}$) and the amplitude error ($< \SI{2}{\percent}$) would have insignificant impact for the sensitivity of the booster. Analogous results are obtained also for other equidistant disk spacings between \SI{6}{\milli\metre} to \SI{8}{\milli\metre}, shifting the boost factor frequency in a range between \SI{22}{\giga\hertz} to \SI{28}{\giga\hertz}.

The correlations in disk spacings illustrate the freedom of a single spacing to still end up with the same electromagnetic response when compensated with the other spacings.
Here an advantage of tuning using multiple parameters is revealed: Phase errors, such as position errors of one disk, can be compensated by moving another disk.
%Therefore, accuracy constrains -- in particular also those derived in Sect.~\ref{sec:sim:non-ideal} -- most likely be loosened considering such a tuning algorithm.
The corresponding uncertainties on the boost factor introduced by the optimization scheme outlined in Fig.~\ref{fig:pop:tuning}\,(c) make this point explicit.
%Therefore, it is currently being investigated how such a reoptimization  sec.~\ref{sec:sim}
	
	\end{comment}
